The star formation histories of galaxies in the Sloan Digital Sky Survey

We present the results of a MOPED analysis of ~3 x 10^5 galaxy spectra from the Sloan Digital Sky Survey Data Release Three (SDSS DR3), with a number of improvements in data, modelling and analysis compared with our previous analysis of DR1. The improvements include: modelling the galaxies with theoretical models at a higher spectral resolution of 3\AA; better calibrated data; an extended list of excluded emission lines, and a wider range of dust models. We present new estimates of the cosmic star formation rate, the evolution of stellar mass density and the stellar mass function from the fossil record. In contrast to our earlier work the results show no conclusive peak in the star formation rate out to a redshift around 2 but continue to show conclusive evidence for `downsizing' in the SDSS fossil record. The star formation history is now in good agreement with more traditional instantaneous measures. The galaxy stellar mass function is determined over five decades of mass, and an updated estimate of the current stellar mass density is presented. We also investigate the systematic effects of changes in the stellar population modelling, the spectral resolution, dust modelling, sky lines, spectral resolution and the change of data set. We find that the main changes in the results are due to the improvements in the calibration of the SDSS data, changes in the initial mass function and the theoretical models used.

==> referee_reply.tex <==
Reply:

We thank the referee for his recommendations, and apologize for the
slow response: further analysis of our data led to the discovery of
two normalization errors in our mass calculations. Although these
two fortuitously (almost) cancel one another out, full investigation
of all possible ramifications of this coupled with the production of
the new SFR/model choice figure took longer than expected.

> My main concern is about the origin of the differences between the
> present analysis and other studies by the same group. Indeed, in this
> paper the authors do not find a significant peak in the SFR out to a
> redshift around 2. In section 3.2 they write that later in the paper
> they will analyze a subset of the data to determine which changes are
>  responsible for the modifications in the results. In section 4 they
> examine how SF fractions vary with different model assumptions
> showing, for example, the impact of different SSP models. But since
> all the discussion in this section is on fractional star formation,
> in the galaxy rest-frame, it is not clear what is the impact of
> different assumptions on the SF history of the universe; in
> particular, it is not clear for me if changes in SSP alone are able
> to 'remove' the low-redshift peak or other factors are also
> important. I suggest that the authors address this issue explicitly
> in section 4, by considering an equivalent of figure 6, but showing
> now the SFR, like in figure 2, for different model assumptions.

We have added this figure and rewritten section 4 to reflect the
changes to the SFF and SFR from different model choices.

>> section 2.1
> - Since the lower redshift limit of the sample, z=0.01, is very
> small, a natural concern is whether or in what extension the results
> -for example, the stellar populations- are affected by an aperture
> bias. For example, Kewley, Jansen & Geller (2005) argue that SDSS
> galaxies should be selected with z>0.04 to minimize aperture effects
> in spectral measurements. This is a issue that should be addressed by
> the authors (not necessarily in this section).

In order to investigate the effect of our redshift cut we have used
samples with various redshift cut offs from 0.001 to 0.05 (see
section 3.1). Although these systematically shift the normalization
slightly, we seen no effect on the shape of the recovered star
formation history. Comment added to this effect.

> - More information should be provided on the sample: How many
> galaxies are in the sample? What is the typical rest-frame wavelength
> range analyzed?

Added.

> - There are some errors in Table 1: where is NI is [NII] and the
> first occurrence of NII should be Halpha. I recommend the adoption of
> the usual designation of forbidden lines with brackets, i.e., [NII]
> instead of NII, etc.

Changed.

> - typos: * 2nd. paragraph: hubble-flow -> Hubble-flow * 3rd.
> paragraph: adsorption -> absorption

Changed.

>> section 2.3
> - I think the reader will appreciate to have more information about
> the 11 time bins adopted in this work. Could you be more specific and
> even list them? (or refer to a figure where they appear).

Text clarified and a list of ages in Gyr added.

> - The only mention to metallicity in this section states that it can
> vary independently in each time bin. This is very ambiguous. Bruzual
> & Charlot (2003) present models for 6 different metallicities. Since
> the number of parameters is 23 (two for each time bin and one for the
> dust), I understand that metallicity does not appear as an
> independent parameter or because a single value was adopted (for all
> bins or for each bin?) or because its evolution is treated
> consistently by a chemical evolution model. Anyway, whatever is the
> case, this issue should be clarified in the text.

Clarified - the metallicity of each bin is allowed to vary
constrained only by the metallicities available in the models. The 2
parameters per bin are the fraction of the spectrum contributed by
that population and the metallicity of that population.

>> section 2.4
> - typo: page 4, 4 lines above eq. 2: evolution of the star ->
> evolution of the galaxy

Fixed.

> - for consistency of the notation, eq. 3 should be changed: * \mu_v
> -> \mu_{i,z} * r -> r_{i,z} * r^2_{50} -> r^2_{50,i}

Fixed.

> - typo: just below eq. 3:  petrosian -> Petrosian

Fixed.

> - Due to technical limitations in the assignment of fibres to targets
> closer than 55 arcmin in the sky, a fraction of galaxies are not
> observed (Stoughton et al. 2002), albeit this problem is more severe
> in high-density regions. Were the densities corrected for this
> effect? Since this problem affects density estimates, the authors
> should comment on the impact of this type of incompleteness in their
> results. I wonder whether the correction by this effect will not help
> to put the SFR results shown in fig. 2 (showing several points below
> the other estimates) more in line with the results of other groups.

The coverage has been corrected, note to this affect added in the
text.


>> section 3.1
> - R is lost in the end of the first paragraph of this section;
> introduce it when mentioning the recycling fraction for the first
> time, in the middle of this paragraph.

Fixed.

> - figure 1: * typo in the y-label of figure 1: Mpc^{-1} ->  Mpc^{-3}

Fixed.

> * why vertical bars with systematic errors were not plotted? This is
> mentioned in section 3.2.

The error bars are entirely correlated. We provide them in the table
as estimates for single points.

>* why only 7 out of 11 time bins were
> plotted?

The time bins plotted in the SFR are the result of shifting the rest
frame star formation histories (which are of course redshift
dependent) to a common set based at z=0. This means that any galaxy
can only contribute to a bin at a greater redshift than that at
which it is observed from earth. In order to remove complications of
extrapolation in partly-contributing bins we only allow galaxies to
contribute to bins whose minimum redshift is greater than that of
the galaxy. In addition, to remove any concern of individual
erroneous star formation histories distorting the results, we only
use bins which have greater than a thousand galaxies contributing.

Note added in the text.

>* I belive that the caption of figure 1 would be more
> readable if the reference to symbol colours appear before the sample
> name.

Fixed.

> - Table 2 is not mentioned in the text. Please, do it, explaining the
>  meaning of Min and Max Density as well.

Added and clarified the meaning of min and max densities in the
context of the approximate systematic errors.

>> section 3.2
> - figure 2: * the same suggestion I made on the caption of fig. 1
> applies here. * why only two bins at z> 1 are shown?

As before.

> - title of table 3: The SFR derived... -> The SFR density derived...

Fixed.

>> section 3.3
> - Schechter fit: in the text appears M^* = 1.017 10^10 M_sun, whereas
> in figure 3 appears M^* = 1.017 10^11 M_sun; fix the wrong number.

Fixed.

> - figure 3: explain the meaning of the red line in the caption.

Done - it is the best Schechter fit solution.

> - the authors adopt two different notations in this section to refer
> to statistical and systematic errors; I recommend to uniformize the
> notation.

Fixed.

> - the systematic error quoted for Omega_b* is 0.1. Is it correct? I
> suspect that the correct value is 0.1 x 10^-3.

Fixed.

>> section 3.5
> - figure 5:  typos in the caption: * panes -> panels * it is also
> missing a closing parenthesis in the last line: ...redshift range).

Fixed.

> - the authors discuss the strong residuals red-ward of the Mg line at
> 5176A, suggesting that they might be part of a feature between
> rest-frame 5200-6500A. Why this wavelength range? Examining fig. 5, I
> see this excess extending at most to 5900A.

Corrected to 5900A.

>> section 4.1
> - In this section, the number of galaxies selected for the analysis
> is 767, whereas in section 4.3 appears another number: 832. What is
> the correct number?

767 of the 808 galaxies used in the Main Galaxy Catalogue would have
been selected for the analysis. This has been clarified in the text.
We have removed some galaxies which have instrumental faults in the
spectra or obviously erroneous redshifts.

>> section 4.3
> - The authors argue that for bins 5 and 7 the deviations between DR3
> and DR1 are large. What about bin 8? The deviation in this bin seems
> larger than in the others.

We have rewritten this section

>> section 4.7
> - typo in the 11th line: panel c) -> panel 6e

Fixed.

> - the authors argue
> that there is virtually no differences for the youngest bins; this is
> not what I see in panel 6e: the amplitude of the differences in the
> two youngest bins are larger than in the second bin.

The deviation between the youngest bins is almost covered by the
bootstrap errors, while the errors on the older populations are
tiny. Hence the differences at the old end are more important.
Clarified in text.

> - typo in the
> 4th line before the end of this section: choose between 'yield' and
> 'allow'.

Fixed

>> section 4.8
> - typo in the 5th line before the end of the section: emisssion ->
> emission

Fixed.

>> section 5
> - typo in the caption of figure 8: panes -> panels

Fixed.

>> section 6
> - I really do not understand the first item of the conclusions
> because, from figure 6, the impact of different stellar population
> models on the SFF (and probably also on the SFR) seems to be much
> more important than spectral calibration or IMF changes. Indeed,
> changes in the dust model seem much more significant than changes in
> the IMF. - in the last item, the proposed avenue for investigation of
> the continuum should be more informative.

The new figure suggested by the referee has clarified this. Although
the differences on normalised recovered SFF are small for the IMF
and spectral calibration, when propagated through the mass and V_max
pipelines they cause large differences to the SFR.

Last statement regarding continuum removed.

